Towards Real Time Egocentric Segment Captioning for The Blind and Visually Impaired in RGB-D Theatre Images

In recent years, image captioning and segmentation have emerged as crucial tasks in computer vision, with applications ranging from autonomous driving to content analysis. Although multiple solutions have emerged to help blind and visually impaired people move around their environment, few are applications that help them understand and rebuild a scene in their minds through text. Most built models focus on helping users move and avoid obstacles, restricting the number of environments blind and visually impaired people can be in. In this paper, we will propose an approach that helps them understand their surroundings using image captioning. The particularity of our research is that we offer them descriptions with positions of regions and objects regarding them (left, right, front), as well as positional relationships between regions, while we aim to give them access to theatre plays by applying the solution to our TS-RGBD dataset.

==> litteraturebackground.tex <==
Before delving into the content of this paper, we will first establish precise definitions for key terms that are essential to our research.


\subsection{Image Captioning}
Image captioning serves as a bridge between computer vision and natural language processing, wherein an intelligent system takes an image as input and generates a corresponding text description that accurately portrays the content depicted in the image.

The generated text takes the form of one sentence for the whole image which is known as sentence captioning, it could be a paragraph: paragraph captioning, or a sentence for each region of interest which is defined as dense captioning.

\subsection{Image Segmentation}
Image segmentation is a computer vision task that involves dividing an image into multiple regions or segments based on certain characteristics such as colour, texture, or object boundaries. The goal of image segmentation is to partition an image into meaningful and semantically coherent regions to facilitate further analysis, understanding, or manipulation of the image's content. Each segment typically corresponds to a specific object or region of interest within the image, allowing for a more detailed and precise analysis of the visual information.

There are three types of segmentation: \textit{i) Instance segmentation:} which provides individual salient objects within an image, \textit{ii) Semantic Segmentation:} it labels each pixel in an image with a class, objects belonging to the same class have the same label, \textit{Panoptic Segmentation:} combines instance and semantic segmentation by assigning a label an id for each pixel.

\subsection{Depth Images}
A depth image is an image that provides information about the distance in millimeters between each pixel and the sensor used to capture the scene. It gives a more accurate understanding of the spatial structure and geometry of the environment. 

When utilising a depth sensor to capture an image, the output includes the RGB image as well as an additional fourth channel that represents the distance of each pixel from the camera. This fourth channel provides depth information.

\subsection{Egocentric Description}
Egocentric captions, as defined in our study, refer to textual descriptions of regions of interest in an image that includes directional information.

This directional information indicates the side to which the user should face to observe the specified region. The purpose of these descriptions is to provide users, particularly the blind and visually impaired, with valuable information about their position in the scene. This enables them to locate objects in their environment or mentally construct a map of their surroundings.

\subsection{Positional relationships between Regions}
Positional relationships between objects refer to the spatial positions of each region or object regarding other ones.

These relationships are determined based on the overlapping of objects, allowing us to use their coordinates to ascertain if an object or region is behind, next to, above, on top of, or in proximity to another region.


\subsection{Region of Interest}
A region of interest (ROI) in an image refers to a specific portion or area within the image that is of particular significance or focus. It is a subset of the image that is selected or defined based on its relevance to the task or analysis being performed.

It is either one or multiple objects, one or many persons, or animals.

In our study, we will refer to segments as regions of interest.
